Transit Detection of a "Starshade" at the Inner Lagrange Point of an Exoplanet

All water-covered rocky planets in the inner habitable zones of solar-type stars will inevitably experience a catastrophic runaway climate due to increasing stellar luminosity and limits to outgoing infrared radiation from wet greenhouse atmospheres. Reflectors or scatterers placed near Earth's inner Lagrange point (L1) have been proposed as a 'geo-engineering" solution to anthropogenic climate change and an advanced version of this could modulate incident irradiation over many Gyr or "rescue" a planet from the interior of the habitable zone. The distance of the starshade from the planet that minimizes its mass is 1.6 times the Earth-L1 distance. Such a starshade would have to be similar in size to the planet and the mutual occultations during planetary transits could produce a characteristic maximum at mid-transit in the light-curve. Because of a fortuitous ratio of densities, Earth-size planets around G dwarf stars present the best opportunity to detect such an artifact. The signal would be persistent and is potentially detectable by a future space photometry mission to characterize transiting planets. The signal could be distinguished from natural phenomenon, i.e. starspots or cometary dust clouds, by its shape, persistence, and transmission spectrum.

==> setup.tex <==
%% For anyone who downloaded my source file from arxiv:
%% I stole most of this setup.tex from a paper by Peter .K.G. Williams, but I made a bunch of edits to satisfy my own needs. You might check his paper out (http://arxiv.org/abs/1409.4411) for the original source file or contact him if you have any questions, since I don't really understand how some of these things work. 
%One cool thing it does is you can define an object, just that when someone clicks on the pdf it will link to simbad. I could never quite get this to work, probably because you have to get the text exactly right and my motivation for getting it to work was not super high. 


% basic packages
\usepackage{amsmath,amssymb}
\usepackage[breaklinks,colorlinks,urlcolor=blue,citecolor=blue,linkcolor=blue]{hyperref}
\usepackage{epsfig}    
\usepackage{graphicx}    
\usepackage{lineno}
\usepackage{natbib}
\usepackage{bigints}
\usepackage[outdir=./]{epstopdf}



% font stuff
\usepackage[T1]{fontenc}
\pwifjournal\else
  \usepackage{microtype}
\fi


% emulateapj has overly conservative figure widths, I think because some
% people's figures don't have good margins. Override.
\pwifjournal\else
  \makeatletter
  \renewcommand\plotone[1]{%
    \centering \leavevmode \setlength{\plot@width}{0.95\linewidth}
    \includegraphics[width={\eps@scaling\plot@width}]{#1}%
  }%
  \makeatother
\fi


% My amazing object-referencing system!
%
% \MakeObj[shortname]{ident}{url-escaped name}{formal name}
%    defines an object
% \MakeTrunc{ident}{truncname}
%    defines a truncated name for a blended object (e.g. LP 349-25 *AB*)
%
% \obj{ident}:  link using standard/short name
% \objf{ident}: link using formal/full name
% \objt{ident}: link using the truncated name
%
% Links are \object{} commands if in journal mode, links to Simbad otherwise.
%
% Under the hood:
%
% \pkgwobj@c@<ident> turns its argument into an appropriate link for the object
% \pkgwobj@f<ident>  expands into the formal/full name of the object
% \pkgwobj@s<ident>  expands into the standard/short name of the object

\makeatletter

\newcommand\@simpfx{http://simbad.u-strasbg.fr/simbad/sim-id?Ident=}

\newcommand\MakeObj[4][\@empty]{% [shortname]{ident}{url-escaped}{formalname}
  \pwifjournal%
    \expandafter\newcommand\csname pkgwobj@c@#2\endcsname[1]{\protect\object[#4]{##1}}%
  \else%
    \expandafter\newcommand\csname pkgwobj@c@#2\endcsname[1]{\href{\@simpfx #3}{##1}}%
  \fi%
  \expandafter\newcommand\csname pkgwobj@f#2\endcsname{#4}%
  \ifx\@empty#1%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#4}%
  \else%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#1}%
  \fi}%

\newcommand\MakeTrunc[2]{% {ident}{truncname}
  \expandafter\newcommand\csname pkgwobj@t#1\endcsname{#2}}%

\newcommand{\obj}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@s#1\endcsname}%
  \fi}
\newcommand{\objf}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@f#1\endcsname}%
  \fi}
\newcommand{\objt}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@t#1\endcsname}%
  \fi}

\makeatother


% Evil magic to patch natbib to only highlight the year paper refs, not the
% authors too; as seen in ApJ. From
% http://tex.stackexchange.com/questions/23227/.

\pwifjournal\else
  \usepackage{etoolbox}
  \makeatletter
  \patchcmd{\NAT@citex}
    {\@citea\NAT@hyper@{%
       \NAT@nmfmt{\NAT@nm}%
       \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
       \NAT@date}}
    {\@citea\NAT@nmfmt{\NAT@nm}%
     \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}
  \patchcmd{\NAT@citex}
    {\@citea\NAT@hyper@{%
       \NAT@nmfmt{\NAT@nm}%
       \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
         {\@citeb\@extra@b@citeb}%
       \NAT@date}}
    {\@citea\NAT@nmfmt{\NAT@nm}%
     \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
    {}{}
  \makeatother
\fi


% Object data
\MakeObj{n33370}{NLTT\%2033370}{NLTT~33370\,AB}
\MakeTrunc{n33370}{NLTT~33370}
\MakeObj{tvlm}{TVLM\%20513-46546}{TVLM~513--46546}

% utility



\newcommand{\vdag}{(v)^\dagger}
\newcommand{\oxygen}{O$_2$}
\newcommand{\water}{H$_2$O}
\newcommand{\kep}{{\it Kepler }}
\newcommand{\logg}{$log~g$ }
\newcommand{\metal}{[M/H]}
\newcommand{\um}{$\mu$m}
\newcommand{\fbol}{$F_{\mathrm{bol}}$}
\newcommand{\mbol}{$m_{\mathrm{bol}}$}
\newcommand{\Mbol}{$M_{\mathrm{bol}}$}
\newcommand{\rapsq}{$R_{ap}^2$}
\newcommand{\rchisq}{$\chi^2_{\nu}$}
\newcommand{\hipp}{{\it Hipparcos}}


\newcommand\aafd{erg~s$^{-1}$~cm$^{-2}$~\AA$^{-1}$} % "AAngstrom flux density"
\newcommand\amlt{$\alpha_{\rm MLT}$} % convective mixing length parameter
\newcommand\apx{\ensuremath{\sim}}
\newcommand\cgsflux{erg~s$^{-1}$~cm$^{-2}$}
\newcommand\cgslum{erg~s$^{-1}$}
\newcommand\chandra{\textit{Chandra}}
\newcommand\citeeg[1]{\citep[\eg,][]{#1}}
\newcommand\cps{ct~s$^{-1}$}
\newcommand\dd{\ensuremath{\text{d}}}
\newcommand\eg{\textit{e.g.}}
\newcommand\etal{\textit{et~al.}}
\newcommand\ewha{\ensuremath{\text{EW}(\ha)}}
\newcommand\fig[1]{Figure~\ref{f.#1}}
\newcommand\ha{{\ensuremath{\text{H}\alpha}}}
\newcommand\I{\mathcal{I}}
\newcommand\ie{\textit{i.e.}}
\newcommand\kms{km~s$^{-1}$}
\newcommand\ls{L$_\odot$}
\newcommand\mj{M$_\text{J}$}
\newcommand\ms{M$_\odot$}
\newcommand\nupk{\ensuremath{\nu_\text{pk}}}
\newcommand\percc{cm$^{-3}$}
\newcommand\rcs{\ensuremath{\chi_r^2}}
\newcommand\rj{R$_\text{J}$}
\newcommand\sect[1]{Section~\ref{s.#1}}
\newcommand\sherpa{\textsf{Sherpa}}
\newcommand\sti{Stokes~$I$}
\newcommand\stiv{Stokes~$I$ and~$V$}
\newcommand\stv{Stokes~$V$}
\newcommand\swift{\textit{Swift}}
\newcommand\tb{\ensuremath{T_\text{b}}}
\newcommand\tbl[1]{Table~\ref{t.#1}}
\newcommand\feh{\ensuremath{\text{[Fe/H]}}}
\newcommand\teff{\ensuremath{T_\text{eff}}}
\newcommand\todo[1]{\textcolor{red}{#1}}
\newcommand\ujy{$\mu$Jy}
\newcommand\ujybm{$\mu$Jy~bm$^{-1}$}
\newcommand\uv{$u$\mbox{-}$v$}
\newcommand\vsi{\ensuremath{v \sin i}}

\newcommand\Lb{\ensuremath{L_\text{bol}}}
\newcommand\Lh{\ensuremath{L_\ha}}
\newcommand\Lr{\ensuremath{L_\text{R}}}
\newcommand\sLr{\ensuremath{L_{\nu,\text{R}}}}
\newcommand\Lu{\ensuremath{L_\text{UVW1}}}
\newcommand\Lx{\ensuremath{L_\text{X}}}
\newcommand\Lxf{\ensuremath{L_{\text{X},f}}}
\newcommand\Lxq{\ensuremath{L_{\text{X},q}}}
\newcommand\lb{\ensuremath{[\Lb]}}
\newcommand\lh{\ensuremath{[\Lh]}}
\newcommand\lr{\ensuremath{[\Lr]}}
\newcommand\slr{\ensuremath{[\sLr]}}
\newcommand\lu{\ensuremath{[\Lu]}}
\newcommand\lx{\ensuremath{[\Lx]}}
\newcommand\lxf{\ensuremath{[\Lxf]}}
\newcommand\lxq{\ensuremath{[\Lxq]}}
\newcommand\lhlb{\ensuremath{[\Lh/\Lb]}}
\newcommand\lrlb{\ensuremath{[\Lr/\Lb]}}
\newcommand\lulb{\ensuremath{[\Lu/\Lb]}}
\newcommand\lxlb{\ensuremath{[\Lx/\Lb]}}
\newcommand\lxflb{\ensuremath{[\Lxf/\Lb]}}
\newcommand\lxqlb{\ensuremath{[\Lxq/\Lb]}}
\newcommand\slrlb{\ensuremath{[\sLr/\Lb]}}
\newcommand\slrlx{\ensuremath{[\sLr/\Lx]}}
\newcommand\slrlxf{\ensuremath{[\sLr/\Lxf]}}
\newcommand\slrlxq{\ensuremath{[\sLr/\Lxq]}}

